Scalable Byzantine Reliable Broadcast (Extended Version)

Byzantine reliable broadcast is a powerful primitive that allows a set of processes to agree on a message from a designated sender, even if some processes (including the sender) are Byzantine. Existing broadcast protocols for this setting scale poorly, as they typically build on quorum systems with strong intersection guarantees, which results in linear per-process communication and computation complexity. We generalize the Byzantine reliable broadcast abstraction to the probabilistic setting, allowing each of its properties to be violated with a fixed, arbitrarily small probability. We leverage these relaxed guarantees in a protocol where we replace quorums with stochastic samples. Compared to quorums, samples are significantly smaller in size, leading to a more scalable design. We obtain the first Byzantine reliable broadcast protocol with logarithmic per-process communication and computation complexity. We conduct a complete and thorough analysis of our protocol, deriving bounds on the probability of each of its properties being compromised. During our analysis, we introduce a novel general technique we call adversary decorators. Adversary decorators allow us to make claims about the optimal strategy of the Byzantine adversary without having to make any additional assumptions. We also introduce Threshold Contagion, a model of message propagation through a system with Byzantine processes. To the best of our knowledge, this is the first formal analysis of a probabilistic broadcast protocol in the Byzantine fault model. We show numerically that practically negligible failure probabilities can be achieved with realistic security parameters.

==> plots/evaluation/security.tex <==
\begin{tikzpicture}
\begin{semilogyaxis}[
    title={Security vs. Average sample size},
    xlabel={Average sample size ($S$)},
    ylabel={Security ($\epsilon$)},
    legend pos=north east,
    ymajorgrids=true,
    grid style=dashed,
    width=0.45\textwidth
]
 
\addplot[
	color=palette-0,
    mark=square,
    ]
    coordinates {
    (84, 2.740834e-07)
    (99.75, 6.819240e-09)
    (119.5, 2.910271e-11)
    (136.5, 6.96133e-13)
    (162.75, 1.317256e-16)
    };
    
    \addplot[
	color=palette-1,
    mark=square,
    ]
    coordinates {
    (144.5, 6.06867e-06)
    (176.25, 6.55089e-08)
    (216.75, 1.80321e-10)
    (260, 3.44436e-13)
    (286.5, 8.40084e-15)
    };

    \legend{${\scriptstyle N=2^{10}\; f = 0.10}$, $\scriptstyle N=2^{10}\;f = 0.15$}
 
\end{semilogyaxis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
    title={Security vs. System size},
    xlabel={System size ($N$)},
    ylabel={Security $\rp{\sqrt{\epsilon / \epsilon_0}}$},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    width=0.45\textwidth
]
 
\addplot[
	color=palette-0,
    mark=square,
    ]
    coordinates {
    (1024, 1)
    (2048, 1.826509)
    (3072, 2.655378)
    (4096, 3.332885)
    };
    
    
\addplot[
	color=palette-1,
    mark=square,
    ]
    coordinates {
    (1024, 1)
    (2048, 1.789688)
    (3072, 2.500925)
    (4096, 2.971483)
    };
    
    \addplot[
	color=palette-2,
    mark=square,
    ]
    coordinates {
    (1024, 1)
    (2048, 1.69347)
    (3072, 2.45085)
    (4096, 3.12816)
    };
    
    \addplot[
	color=palette-3,
    mark=square,
    ]
    coordinates {
    (1024, 1)
    (2048, 1.78765)
    (3072, 2.39791)
    (4096, 2.85749)
    };

    \legend{${\scriptstyle f = 0.10\; S = 84}$, ${\scriptstyle f = 0.10\; S = 163}$, ${\scriptstyle f = 0.15\;S = 145}$, ${\scriptstyle f = 0.15\;S = 287}$}
 
\end{axis}
\end{tikzpicture}

==> plots/probabilistic-broadcast/security.tex <==
\begin{tikzpicture}
\begin{semilogyaxis}[
    title={Gossip validity ($N = 1024$)},
    xlabel={Sample size ($G$)},
    ylabel={Failure probability ($\epsilon$)},
    legend pos=south west,
    ymajorgrids=true,
    grid style=dashed,
    width=0.45\textwidth
]
 
\addplot[
	color=palette-0,
    mark=square,
    ]
    coordinates {
    (5, 0.0468971)
    (6, 0.00616465)
    (7, 0.00082308)
    (8, 0.000109936)
    (9, 1.46593e-05)
    (10, 1.95095e-06)
    (11, 2.59128e-07)
    (12, 3.43493e-08)
    (13, 4.54415e-09)
    (14, 5.99956e-10)
    (15, 7.90524e-11)
    (16, 1.03953e-11)
    (17, 1.36422e-12)
    (18, 1.78672e-13)
    };
    
    
\addplot[
	color=palette-1,
    mark=square,
    ]
    coordinates {
    (5, 0.0750802)
    (6, 0.0108075)
    (7, 0.00159513)
    (8, 0.000235931)
    (9, 3.48508e-05)
    (10, 5.13878e-06)
    (11, 7.56299e-07)
    (12, 1.11098e-07)
    (13, 1.6289e-08)
    (14, 2.38374e-09)
    (15, 3.48173e-10)
    (16, 5.07579e-11)
    (17, 7.38554e-12)
    (18, 1.07258e-12)
    (19, 1.55468e-13)
    };
    
\addplot[
	color=palette-2,
    mark=square,
    ]
    coordinates {
    (6, 0.018723)
    (7, 0.00304488)
    (8, 0.000497592)
    (9, 8.12597e-05)
    (10, 1.32489e-05)
    (11, 2.15635e-06)
    (12, 3.50334e-07)
    (13, 5.68154e-08)
    (14, 9.19744e-09)
    (15, 1.48623e-09)
    (16, 2.39728e-10)
    (17, 3.8598e-11)
    (18, 6.20332e-12)
    (19, 9.9516e-13)
    (20, 1.59357e-13)
    };
    
    
\addplot[
	color=palette-3,
    mark=square,
    ]
    coordinates {
    (6, 0.0324293)
    (7, 0.00579829)
    (8, 0.00104639)
    (9, 0.000188894)
    (10, 3.4054e-05)
    (11, 6.12932e-06)
    (12, 1.10135e-06)
    (13, 1.97562e-07)
    (14, 3.53787e-08)
    (15, 6.32472e-09)
    (16, 1.12875e-09)
    (17, 2.01101e-10)
    (18, 3.57672e-11)
    (19, 6.35053e-12)
    (20, 1.12561e-12)
    (21, 1.99166e-13)
    };     

\addplot[
	color=palette-4,
    mark=square,
    ]
    coordinates {
    (6, 0.0562503)
    (7, 0.0110174)
    (8, 0.00219357)
    (9, 0.000437621)
    (10, 8.72306e-05)
    (11, 1.73625e-05)
    (12, 3.45044e-06)
    (13, 6.84614e-07)
    (14, 1.3562e-07)
    (15, 2.68227e-08)
    (16, 5.29646e-09)
    (17, 1.04416e-09)
    (18, 2.05519e-10)
    (19, 4.03861e-11)
    (20, 7.92335e-12)
    (21, 1.55196e-12)
    (22, 3.03492e-13)
    };     

    \legend{$f = 0.00$, $f = 0.05$, $f = 0.10$, $f = 0.15$, $f = 0.20$}
 
\end{semilogyaxis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{semilogyaxis}[
    title={Gossip validity ($N = 8192$)},
    xlabel={Sample size ($G$)},
    ylabel={Failure probability ($\epsilon$)},
    legend pos=south west,
    ymajorgrids=true,
    grid style=dashed,
    width=0.45\textwidth
]
 
\addplot[
	color=palette-0,
    mark=square,
    ]
    coordinates {
    (6, 0.0514704)
    (7, 0.00680596)
    (8, 0.00091692)
    (9, 0.000123815)
    (10, 1.67209e-05)
    (11, 2.25766e-06)
    (12, 3.04757e-07)
    (13, 4.11286e-08)
    (14, 5.54916e-09)
    (15, 7.48522e-10)
    (16, 1.00943e-10)
    (17, 1.36094e-11)
    (18, 1.83441e-12)
    (19, 2.472e-13)
    };
    
    
\addplot[
	color=palette-1,
    mark=square,
    ]
    coordinates {
    (6, 0.0908409)
    (7, 0.0130731)
    (8, 0.00194178)
    (9, 0.000289716)
    (10, 4.32464e-05)
    (11, 6.45465e-06)
    (12, 9.63164e-07)
    (13, 1.43691e-07)
    (14, 2.14316e-08)
    (15, 3.19581e-09)
    (16, 4.76438e-10)
    (17, 7.10118e-11)
    (18, 1.05816e-11)
    (19, 1.57643e-12)
    (20, 2.34798e-13)
    };
    
\addplot[
	color=palette-2,
    mark=square,
    ]
    coordinates {
    (7, 0.0251123)
    (8, 0.00410308)
    (9, 0.000676103)
    (10, 0.000111543)
    (11, 1.84027e-05)
    (12, 3.03557e-06)
    (13, 5.00617e-07)
    (14, 8.25422e-08)
    (15, 1.36066e-08)
    (16, 2.24249e-09)
    (17, 3.695e-10)
    (18, 6.08698e-11)
    (19, 1.00252e-11)
    (20, 1.65078e-12)
    (21, 2.71762e-13)
    };
    
    
\addplot[
	color=palette-3,
    mark=square,
    ]
    coordinates {
    (7, 0.0482708)
    (8, 0.00863774)
    (9, 0.0015701)
    (10, 0.000286165)
    (11, 5.21728e-05)
    (12, 9.51094e-06)
    (13, 1.73349e-06)
    (14, 3.15885e-07)
    (15, 5.75501e-08)
    (16, 1.04827e-08)
    (17, 1.90902e-09)
    (18, 3.47581e-10)
    (19, 6.32721e-11)
    (20, 1.15154e-11)
    (21, 2.09533e-12)
    (22, 3.81186e-13)
    };     

\addplot[
	color=palette-4,
    mark=square,
    ]
    coordinates {
    (7, 0.0935578)
    (8, 0.0181991)
    (9, 0.0036432)
    (10, 0.000733401)
    (11, 0.000147782)
    (12, 2.97794e-05)
    (13, 5.99996e-06)
    (14, 1.20865e-06)
    (15, 2.43425e-07)
    (16, 4.9017e-08)
    (17, 9.86832e-09)
    (18, 1.98634e-09)
    (19, 3.99743e-10)
    (20, 8.04306e-11)
    (21, 1.618e-11)
    (22, 3.25423e-12)
    (23, 6.54384e-13)
    };     

    \legend{$f = 0.00$, $f = 0.05$, $f = 0.10$, $f = 0.15$, $f = 0.20$}
 
\end{semilogyaxis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{semilogyaxis}[
    title={Gossip validity ($N = 65536$)},
    xlabel={Sample size ($G$)},
    ylabel={Failure probability ($\epsilon$)},
    legend pos=south west,
    ymajorgrids=true,
    grid style=dashed,
    width=0.45\textwidth
]
 
\addplot[
	color=palette-0,
    mark=square,
    ]
    coordinates {
    (7, 0.0559772)
    (8, 0.00739694)
    (9, 0.00099765)
    (10, 0.000134924)
    (11, 1.82536e-05)
    (12, 2.46955e-06)
    (13, 3.34099e-07)
    (14, 4.51982e-08)
    (15, 6.11439e-09)
    (16, 8.27126e-10)
    (17, 1.11886e-10)
    (18, 1.51346e-11)
    (19, 2.04715e-12)
    (20, 2.76895e-13)
    };
    
    
\addplot[
	color=palette-1,
    mark=square,
    ]
    coordinates {
    (8, 0.0157051)
    (9, 0.00233295)
    (10, 0.000348508)
    (11, 5.21041e-05)
    (12, 7.79065e-06)
    (13, 1.16485e-06)
    (14, 1.74164e-07)
    (15, 2.60394e-08)
    (16, 3.89307e-09)
    (17, 5.82024e-10)
    (18, 8.70116e-11)
    (19, 1.30077e-11)
    (20, 1.94451e-12)
    (21, 2.90676e-13)
    };
    
\addplot[
	color=palette-2,
    mark=square,
    ]
    coordinates {
    (8, 0.0334044)
    (9, 0.00544519)
    (10, 0.000897848)
    (11, 0.000148321)
    (12, 2.45091e-05)
    (13, 4.05007e-06)
    (14, 6.69252e-07)
    (15, 1.10587e-07)
    (16, 1.82729e-08)
    (17, 3.01926e-09)
    (18, 4.98861e-10)
    (19, 8.24228e-11)
    (20, 1.36177e-11)
    (21, 2.24982e-12)
    (22, 3.71688e-13)
    };
    
    
\addplot[
	color=palette-3,
    mark=square,
    ]
    coordinates {
    (8, 0.0715139)
    (9, 0.012696)
    (10, 0.00230695)
    (11, 0.00042095)
    (12, 7.68682e-05)
    (13, 1.40382e-05)
    (14, 2.56377e-06)
    (15, 4.68204e-07)
    (16, 8.5503e-08)
    (17, 1.56141e-08)
    (18, 2.85128e-09)
    (19, 5.20657e-10)
    (20, 9.50719e-11)
    (21, 1.73597e-11)
    (22, 3.16972e-12)
    (23, 5.78745e-13)
    };     

\addplot[
	color=palette-4,
    mark=square,
    ]
    coordinates {
    (9, 0.0296394)
    (10, 0.00591346)
    (11, 0.00119086)
    (12, 0.000240262)
    (13, 4.84912e-05)
    (14, 9.78732e-06)
    (15, 1.97543e-06)
    (16, 3.98703e-07)
    (17, 8.04686e-08)
    (18, 1.62403e-08)
    (19, 3.27756e-09)
    (20, 6.61449e-10)
    (21, 1.33485e-10)
    (22, 2.69374e-11)
    (23, 5.43588e-12)
    (24, 1.09692e-12)
    (25, 2.21343e-13)
    };     

    \legend{$f = 0.00$, $f = 0.05$, $f = 0.10$, $f = 0.15$, $f = 0.20$}
 
\end{semilogyaxis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{semilogyaxis}[
    title={Gossip validity ($N = 524288$)},
    xlabel={Sample size ($G$)},
    ylabel={Failure probability ($\epsilon$)},
    legend pos=south west,
    ymajorgrids=true,
    grid style=dashed,
    width=0.45\textwidth
]
 
\addplot[
	color=palette-0,
    mark=square,
    ]
    coordinates {
    (8, 0.0607705)
    (9, 0.00801589)
    (10, 0.00108106)
    (11, 0.000146232)
    (12, 1.97882e-05)
    (13, 2.67791e-06)
    (14, 3.62398e-07)
    (15, 4.90427e-08)
    (16, 6.63683e-09)
    (17, 8.98145e-10)
    (18, 1.21543e-10)
    (19, 1.6448e-11)
    (20, 2.22583e-12)
    (21, 3.01211e-13)
    };
    
    
\addplot[
	color=palette-1,
    mark=square,
    ]
    coordinates {
    (9, 0.0188311)
    (10, 0.00279416)
    (11, 0.00041741)
    (12, 6.24181e-05)
    (13, 9.33518e-06)
    (14, 1.39618e-06)
    (15, 2.08816e-07)
    (16, 3.12307e-08)
    (17, 4.67088e-09)
    (18, 6.98577e-10)
    (19, 1.04479e-10)
    (20, 1.56258e-11)
    (21, 2.33696e-12)
    (22, 3.49511e-13)
    };
    
\addplot[
	color=palette-2,
    mark=square,
    ]
    coordinates {
    (9, 0.0444297)
    (10, 0.00721138)
    (11, 0.00118842)
    (12, 0.000196341)
    (13, 3.2451e-05)
    (14, 5.36382e-06)
    (15, 8.86591e-07)
    (16, 1.46545e-07)
    (17, 2.42225e-08)
    (18, 4.00373e-09)
    (19, 6.61774e-10)
    (20, 1.09384e-10)
    (21, 1.80798e-11)
    (22, 2.98837e-12)
    (23, 4.93938e-13)
    };
    
    
\addplot[
	color=palette-3,
    mark=square,
    ]
    coordinates {
    (10, 0.0186189)
    (11, 0.00337568)
    (12, 0.000615813)
    (13, 0.000112467)
    (14, 2.05441e-05)
    (15, 3.75289e-06)
    (16, 6.8556e-07)
    (17, 1.25235e-07)
    (18, 2.28772e-08)
    (19, 4.17906e-09)
    (20, 7.63403e-10)
    (21, 1.39453e-10)
    (22, 2.54741e-11)
    (23, 4.6534e-12)
    (24, 8.5004e-13)
    };     

\addplot[
	color=palette-4,
    mark=square,
    ]
    coordinates {
    (10, 0.0483275)
    (11, 0.00957399)
    (12, 0.00192555)
    (13, 0.000388451)
    (14, 7.8412e-05)
    (15, 1.583e-05)
    (16, 3.19587e-06)
    (17, 6.45205e-07)
    (18, 1.30258e-07)
    (19, 2.62974e-08)
    (20, 5.30906e-09)
    (21, 1.07182e-09)
    (22, 2.16383e-10)
    (23, 4.36843e-11)
    (24, 8.81912e-12)
    (25, 1.78043e-12)
    (26, 3.59436e-13)
    };     

    \legend{$f = 0.00$, $f = 0.05$, $f = 0.10$, $f = 0.15$, $f = 0.20$}
 
\end{semilogyaxis}
\end{tikzpicture}

==> sections/conclusions.tex <==
\section{Conclusions}
\label{section:related}

